IdeaBlocks: Expressing and Reusing Divergent Intents for Graphic Design Exploration using Generative AI

While designers increasingly leverage Generative AI for divergent exploration, current interaction is optimized for convergent refinement, forcing users to specify fixed targets rather than open-ended search spaces. Based on a formative study (N=7), we define the anatomy of Divergent Intent, comprising property, direction, and range, and identified two critical barriers: the lack of mechanisms to explicitly shape the parametric boundaries of exploration and the difficulty of reusing successful search strategies. We present IdeaBlocks, where users can modularize divergent intents into Exploration Blocks. Users can reuse prior intents at multiple levels (block, path, and project) with options for literal or context-adaptive reuse. In our comparative study (N=12), participants using IdeaBlocks explored 2.13 times more images with 12.5% greater visual diversity than the baseline, demonstrating how structured intent expression and reuse support effective divergence. A three-day deployment study (N=6) further revealed how different reuse mechanisms allowed distinct creative strategies, offering design implications for future intent-aware creativity supports.

==> Sections/99-Prompts.tex <==

% \section{Technical Detail}
\appendix
We present the full prompts used in \sysname{}'s pipeline for operationalizing divergent intent. The pipeline consists of six processes: (A) generating design properties from a given topic, (B) translating divergent intent into system-generated suggestions, (C) generating images that incorporate exploration history, (D) organizing exploration history for context-aware reuse, (E) supporting context-adaptive reuse across block, path, and project levels, and (F) recommending exploration directions based on prior exploration. For each stage, we provide the prompt instruction along with representative input-output examples.

\section{Generate a List of Properties}

\begin{prompt}
\obeylines
\setlength{\parindent}{0pt}
\textbf{Prompt Instruction:}

Suggest design exploratory properties based on a given design topic. Provide eight properties to inspire the designer's exploration process. Each property must include three elements: property name, property type, and category. Ensure that each property focuses on only one element.

- Property name: Suggest the name of an important design element to be explored.
- Property type: Either text or image, depending on the most appropriate mode of expression.

\# Output format:
\begin{verbatim}
{
  "outputs": [
    {
      "property_name": "<property_name>",
      "property_type": "<text or image>"
    },
    ...
  ]
}
\end{verbatim}

\# Notes:
- Ensure that the property that needs to be explored first appears first in the list.
- Each property should cover only a single distinct element (e.g., texture or color, not both).
- Consider whether the property is better explored via text or image.
- Always include core properties such as image style.

\vspace{0.5em}
\noindent\hrulefill
\vspace{0.5em}

\textbf{Examples:}

\textbf{Input:} \texttt{A professional mascot character for a laboratory}

\textbf{Output:}
\begin{verbatim}
{
  "outputs": [
    {
      "property_name": "Mascot's Entity",
      "property_type": "text"
    },
    {
      "property_name": "Mascot's Pose",
      "property_type": "text"
    },
    {
      "property_name": "Character Aesthetics",
      "property_type": "text"
    },
    {
      "property_name": "Laboratory Setting",
      "property_type": "text"
    },
    {
      "property_name": "Image Style",
      "property_type": "image"
    },
    {
      "property_name": "Mascot's Clothing",
      "property_type": "text"
    },
    {
      "property_name": "Field of Expertise of the Lab",
      "property_type": "text"
    },
    {
      "property_name": "Safety Gear",
      "property_type": "text"
    }
  ]
}
\end{verbatim}

\textbf{Input:} \texttt{An illustration for a child book cover with a friendly monster}

\textbf{Output:}
\begin{verbatim}
{
  "outputs": [
    {
      "property_name": "World's Landscape",
      "property_type": "text"
    },
    {
      "property_name": "Color Palette",
      "property_type": "image"
    },
    {
      "property_name": "Unusual Structures",
      "property_type": "text"
    },
    {
      "property_name": "Lighting Effects",
      "property_type": "image"
    },
    {
      "property_name": "Atmosphere",
      "property_type": "text"
    },
    {
      "property_name": "Image Style",
      "property_type": "image"
    },
    {
      "property_name": "Fantasy Creatures",
      "property_type": "text"
    },
    {
      "property_name": "Architectural Features",
      "property_type": "text"
    }
  ]
}
\end{verbatim}

\textbf{Input:} \texttt{A drawing of a surreal worlds with fantasy mood}

\textbf{Output:}
\begin{verbatim}
{
  "outputs": [
    {
      "property_name": "Monster's Appearance",
      "property_type": "text"
    },
    {
      "property_name": "Color Palette",
      "property_type": "image"
    },
    {
      "property_name": "Monster's Facial Expression",
      "property_type": "text"
    },
    {
      "property_name": "Background Setting",
      "property_type": "text"
    },
    {
      "property_name": "Image Style",
      "property_type": "image"
    },
    {
      "property_name": "Typography",
      "property_type": "text"
    },
    {
      "property_name": "Symbolic Expression of Monster",
      "property_type": "text"
    },
    {
      "property_name": "Child Character",
      "property_type": "text"
    }
  ]
}
\end{verbatim}
\end{prompt}


\section{Divergent Intent into System-Generated Suggestions}\label{supp:suggestion}
\subsection{Direction Diversification}\label{appendix:suggestionprompt1}\leavevmode\\

\setlength{\parindent}{0pt}
\texttt{\#\# Text-based property}

\begin{prompt}
\obeylines
\setlength{\parindent}{0pt}
\textbf{Prompt Instruction:}

You're an innovative and creative assistant in generating direction alternatives, given the design exploration context. A user is exploring various design alternatives in a design topic. The user's design exploration context will be provided to you to support their exploration process by suggesting various alternatives. You'll be provided with two key pieces of information that define the user's design context. These elements describe the user's design exploration setup, giving a clear foundation for generating alternative directions:

1. Property Name (e.g., "Mascot Attire") - This specifies the aspect of the design that the user wants to explore alternatives for, such as clothing, accessories, or visual characteristics.
2. Direction (e.g., "Hippie") - This indicates the direction or theme that the user wants to diverge from within the property.

\# Task:
Your task is to generate 9 diverging directions. Direction variations must be split into two categories:
1. 4 Sub-directions – Directions that are subtypes of the direction.
2. 5 Unrelated Directions – Variations must be distinct, sharing no semantic similarity with each other.

- Ensure the direction alternatives remain aligned with the property.
- Ensure directional variations use clear, familiar terms and remain concise, avoiding unnecessary details.

\# Output Format
Output should follow the JSON format:
\begin{verbatim}
{
  "outputs": {
    "variations": [
      "<subtype_output_1>",
      "<subtype_output_2>",
      "<subtype_output_3>",
      "<subtype_output_4>",
      "<unrelated_output_1>",
      "<unrelated_output_2>",

      "...",

      "<unrelated_output_5>"
    ]
  }
}
\end{verbatim}

\vspace{0.5em}
\noindent\hrulefill
\vspace{0.5em}

\textbf{Examples:}

\textbf{Input:}
"Property Name: "Mascot Species"
"Direction": "Cat"

\textbf{Output:} 
\begin{verbatim}
{
  "outputs": {
    "variations": [
      "Sphynx", "Persian", "Siamese", "Bengal",
      "Dog", "Parrot", "Dragon", "Kangaroo", "Turtle"
    ]
  }
}
\end{verbatim}

\textbf{Input:}
"Property Name: "Dragon Wings"
"Direction": "Elemental (Fire)"

\textbf{Output:} 
\begin{verbatim}
{
  "outputs": {
    "variations": [
      "Lava", "Blaze", "Inferno", "Ember",
      "Crystal", "Feathered", "Mechanical", "Insect", "Bat"
    ]
  }
}
\end{verbatim}

\textbf{Input:}
"Property Name: "Mascot Attire"
"Direction": "Hippie"

\textbf{Output:} 
\begin{verbatim}
{
  "outputs": {
    "variations": [
      "Bohemian", "Tie-Dye", "Flower Child", "Vintage 70s",
      "Formal", "Sporty", "Steampunk", "Futuristic", "Pirate"
    ]
  }
}
\end{verbatim}

\textbf{Input:}
"Property Name: "Building Facade"
"Direction": "Cyberpunk"

\textbf{Output:} 
\begin{verbatim}
{
  "outputs": {
    "variations": [
      "Neon-lit", "High-tech", "Dystopian", "Industrial",
      "Victorian", "Art Deco", "Organic", "Mediterranean", "Minimalist"
    ]
  }
}
\end{verbatim}

\end{prompt}

\setlength{\parindent}{0pt}
\texttt{\#\# Image-based property}

\begin{prompt}
\obeylines
\setlength{\parindent}{0pt}
\textbf{Prompt Instruction:}

You're an innovative and creative assistant in generating direction alternatives, given the design exploration context. A user is exploring various design alternatives in a design topic. The user's design exploration context will be provided to you to support their exploration process by suggesting various alternatives. You'll be provided with two key pieces of information that define the user's design context. These elements describe the user's design exploration setup, giving a clear foundation for generating alternative directions:

1. Property Name (e.g., "Image Style") - This specifies the visual aspect of the design that the user wants to explore alternatives for, such as style, color, and texture.
2. Direction (e.g., "Vintage") - This indicates the direction or theme that the user wants to diverge from within the property. 

\# Task:
Your task is to generate 9 alternative directions. Direction variations must be split into two categories:
1. 4 Sub-directions – Directions that are decomposed subtypes of the direction.
2. 5 Unrelated Directions – Variations must be distinct, sharing no semantic similarity with each other.

- Ensure the direction alternatives remain aligned with the property.
- Ensure directional variations use clear, familiar terms and remain concise, avoiding unnecessary details.

\# Output Format
Output should follow the JSON format:
\begin{verbatim}
{
  "outputs": {
    "variations": [
      "<subtype_output_1>",
      "<subtype_output_2>",
      "<subtype_output_3>",
      "<subtype_output_4>",
      "<unrelated_output_1>",
      "<unrelated_output_2>",

      "...",

      "<unrelated_output_5>"
    ]
  }
}
\end{verbatim}

\vspace{0.5em}
\noindent\hrulefill
\vspace{0.5em}

\textbf{Examples:}

\textbf{Input:}
"Property Name: "Color Scheme"
"Direction": "Pastel"

\textbf{Output:} 
\begin{verbatim}
{
  "outputs": {
    "variations": [
      "Soft Pastel", "Muted Pastel", "Bright Pastel", "Earthy Pastel",
      "Neon", "Monochrome", "Earth Tones", "Primary Colors", "High Contrast"
    ]
  }
}
\end{verbatim}

\textbf{Input:}
"Property Name: "Image Style"
"Direction": "Vintage"

\textbf{Output:} 
\begin{verbatim}
{
  "outputs": {
    "variations": [
      "Retro Vintage", "Classic Vintage", "Industrial Vintage", "Rustic Vintage",
      "Minimalist", "Surreal", "Futuristic", "Abstract", "Pop Art"
    ]
  }
}
\end{verbatim}

\end{prompt}

\subsection{Suggestion Options Generation}\label{appendix:suggestionprompt2}\leavevmode\\

\setlength{\parindent}{0pt}
\texttt{\#\# Text-based property}

\begin{prompt}
\obeylines
\setlength{\parindent}{0pt}
\textbf{Prompt Instruction:}

You're an assistant in generating text alternatives, given the design exploration context. A user is exploring various design alternatives in a design topic. The user's design exploration context will be provided to you to support their exploration process by suggesting various alternatives. You'll be provided with five key pieces of information that define the user's design context. These elements describe the user's design exploration setup, giving a clear foundation for generating alternative suggestions:

1. Design Topic (e.g., "A cute mascot character for a children's book") - This sets the overarching theme or context for the design.
2. Current Settings (e.g., "Character Entity: Fox") - These are the specific elements the user has already chosen for the design, providing context for the kind of element they want to fix in their exploration.
3. Property Name (e.g., "Mascot Attire") - This specifies the aspect of the design that the user wants to explore alternatives for, such as clothing, accessories, or visual characteristics.
4. Direction (e.g., "Hippie") - This indicates the specific direction or theme that the user wants the property to fit into.

\# Task:
Your task is to generate 10 similar variations for the specified direction within the chosen design property.  Directional variations should consistently use terminology aligned with the original input direction.

- Ensure directional variations are clear and concise.
- Ensure the direction alternatives adhere with the provided design exploration context(Current Settings and Property).
- Directional variations should remain consistent with the input direction, ensuring they are standard, predictable, and familiar.
- Ensure directional variations are diverse and distinctly different from one another.
- Ensure directional variations use easy, familiar terms, avoiding unnecessary elements.

\# Output Format
Output should follow the JSON format:
\begin{verbatim}
{
  "outputs": {
      "literal_variations": [
        "<output_1>",
        "<output_2>",
        "...",
        "<output_10>"
    ]
  }
}
\end{verbatim}

\vspace{0.5em}
\noindent\hrulefill
\vspace{0.5em}

\textbf{Examples:}

\textbf{Input:}
Design Topic: "A mystical creature for a fantasy novel cover"
Current Settings: ["Creature Type: Dragon", "Dragon Color: Dark Blue"]
Property Name: "Dragon Wings"
Direction: "Elemental (Fire)"

\textbf{Output:} 
\begin{verbatim}
{
  "outputs": {
    "literal_variations": [
      "Blazing Flame Trails", "Lava-Inspired Ripples",
      "Ember Flicker Patterns", "Inferno Edge Design",
      "Fiery Vein Details", "Volcanic Glow Highlights",
      "Scorch-Inspired Textures", "Searing Heat Streaks",
      "Crimson Spark Traces", "Radiant Flame Outlines"
    ]
  }
}
\end{verbatim}

\textbf{Input:}
Design Topic: "A cute mascot character for a children's book"
Current Settings: ["Character Entity: Fox", "Mascot Personality: Playful"]
Property Name: "Mascot Attire"
Direction: "Hippie"

\textbf{Output:} 
\begin{verbatim}
{
  "outputs": {
    "literal_variations": [
      "Tie-Dye Shirt", "Fringed Vest",
      "Flower Crown", "Peace Sign Necklace",
      "Patchwork Pants", "Crochet Hat",
      "Beaded Accessories", "Round Glasses",
      "Sandals with Beads", "Embroidered Jacket"
    ]
  }
}
\end{verbatim}

\textbf{Input:}
Design Topic: "A futuristic cityscape for a video game"
Current Settings: ["Building Type: Skyscraper"]
Property Name: "Building Facade"
Direction: "Cyberpunk"

\textbf{Output:} 
\begin{verbatim}
{
  "outputs": {
    "literal_variations": [
      "Neon Grid Patterns", "Holographic Advertisements",
      "LED Matrix Panels", "Translucent Digital Displays",
      "Pulsating Light Strips", "Reflective Metal Surfaces",
      "Augmented Reality Facades", "Fluorescent Tube Designs",
      "Virtual Banner Walls", "Laser-Cut Glass Sections"
    ]
  }
}
\end{verbatim}

\end{prompt}

\setlength{\parindent}{0pt}
\texttt{\#\# Image-based property}

\begin{prompt}
\obeylines
\setlength{\parindent}{0pt}
You are an advanced AI assistant specializing in generating highly effective prompts for text-to-image models. Your task is to create multiple short prompts that illustrate a specified visual concept, ensuring diversity between prompts.
Create 5 distinct prompts that effectively illustrate the given visual concept.

\# Steps
1. Identify the core characteristics of the visual concept(e.g., texture, composition, lighting, artistic style, subject matter).
2. Generate diverse prompts that accurately illustrates the property concept.

\# Guidelines
- Keep final prompts well-structured and short.
- Avoid Repetition - Do not reuse similar structures or elements across different prompts.
- Ensure Safety - Each prompt should not contain text that is not allowed by the safety system.

\# Input Format
\begin{verbatim}
## Visual Property: {image_property}
## Visual Concept: {property_value}
\end{verbatim}
\end{prompt}

\section{Image Generation Pipeline}

\subsection{Property Extraction}\label{appendix:generationprompt1}\leavevmode

\begin{prompt}
\obeylines
\setlength{\parindent}{0pt}

You are an advanced AI assistant specializing in image analysis, providing detailed descriptions of specific visual properties within a given image.
Your goal is to deconstruct and articulate each visual property into its key aspects, ensuring the output is adaptable to effective visual property transfer.

\# Task
Analyze the provided image and generate a **concrete description** for each specific visual property in the property list.

\# Guidelines
- Focus on the key visual characteristics associated with the visual properties: \{property\_list\}.
- Each description must be a concise, objective, short paragraph, emphasizing intricate details that characterize the visual property.
- Response must include descriptions for all visual properties in:
\{property\_list\}

\# Input Format
\begin{verbatim}
## Visual Properties: {property_list}
\end{verbatim}

\end{prompt}

\subsection{Prompt creation}\label{appendix:generationprompt2}\leavevmode

\begin{prompt}
\obeylines
\setlength{\parindent}{0pt}
\textbf{Prompt Instruction:}

You are an advanced AI specializing in crafting text-to-image prompts by seamlessly integrating specific visual properties.

\# Task
Your goal is to create a well-structured, descriptive text-to-image prompt that accurately represents the provided visual property descriptions.

\# Steps
1. For each visual property description, extract the key elements that are enticed to the specific visual property. Eliminate irrelevant descriptions.
2. Compose a well-structured text-to-image prompt that effectively combines the key elements of each visual property, to ensure all extracted elements are clearly reflected in the output image.

\# Guidelines
- The final prompt must emphasize the most recent visual property, while comprising the remainig properties holistically.
- Do not introduce any additional details beyond what is explicitly provided.  
- The prompt must be structured to maximize the generation alignment with the intended image.

\# Input Format
\begin{verbatim}
## Visual property descriptions ##
### Most recent visual property
{current_property_caption_text}
### Remaining visual properties
{prev_properties_caption_text}
\end{verbatim}

\# Output Format
Your response should contain only the fully refined, well-structured
text-to-image prompt.
\end{prompt}

\section{Exploration History Organization}
This prompt is used to organize the exploration history displayed in \sysname{}'s sidebar, allowing users to browse and retrieve previously created Exploration Blocks.

\begin{prompt}
\obeylines
\setlength{\parindent}{0pt}
\textbf{Prompt Instruction:}

Identify the most relevant exploration log from a list of previous exploration logs by comparing it to the latest exploration log.
Compare the "direction" fields to determine the thematic similarity between logs. Consider logs with similar themes as more relevant. Return the "id" of the most thematically similar log or "None" if no relevant match is found.

\# Examples:
Input1:
- Previous Exploration Logs:
\begin{verbatim}
[
    {"id": "1", "direction": "hippie attires"},
    {"id": "2", "direction": "classic attires"}
]
\end{verbatim}
- New Exploration Log: student's attires

Output1:
2
(Because "student attires" are closer to "classic attires.")

Input2:
- Previous Exploration Logs:
\begin{verbatim}
[
    {"id": "1", "direction": "avant-garde art"},
    {"id": "2", "direction": "futuristic design"}
]
\end{verbatim}
- New Exploration Log: medieval architecture

Output2:
None
(Because "medieval architecture" does not closely resemble either "avant-garde art" or "futuristic design.")

\# Notes:
- Previous exploration logs are in chronological order. Therefore, you can give more weight to the later entries in the log, as they are more recent and highly likely to be related to the current log.

\vspace{0.5em}
\noindent\hrulefill
\vspace{0.5em}

\textbf{Examples:}

\textbf{Input:}
- Previous Exploration Logs:
\begin{verbatim}
[
    {"id": "1", "direction": "animal",
    {"id": "2", "direction": "magical animal"}
    {"id": "3", "direction": "flying magical animal"}
    {"id": "4", "direction": "sea creatures"}
]
\end{verbatim}
- New Exploration Log: deep sea creatures

\textbf{Output:} 4

\textbf{Input:}
- Previous Exploration Logs:
\begin{verbatim}
[
    {"id": "1", "direction": "animal",
    {"id": "2", "direction": "magical animal"}
    {"id": "3", "direction": "flying magical animal"}
    {"id": "4", "direction": "sea creatures"}
]
\end{verbatim}
- New Exploration Log: unicorn

\textbf{Output:} 2

\textbf{Input:}
- Previous Exploration Logs:
\begin{verbatim}
[
    {"id": "1", "direction": "animal",
    {"id": "2", "direction": "magical animal"}
    {"id": "3", "direction": "flying magical animal"}
    {"id": "4", "direction": "sea creatures"}
]
\end{verbatim}
- New Exploration Log: dragon

\textbf{Output:} 3

\textbf{Input:}
- Previous Exploration Logs:
\begin{verbatim}
[
    {"id": "1", "direction": "animal",
    {"id": "2", "direction": "magical animal"}
    {"id": "3", "direction": "flying magical animal"}
    {"id": "4", "direction": "sea creatures"}
]
\end{verbatim}
- New Exploration Log: mammal

\textbf{Output:} 1

\textbf{Input:}
- Previous Exploration Logs:
\begin{verbatim}
[
    {"id": "1", "direction": "animal",
    {"id": "2", "direction": "magical animal"}
    {"id": "3", "direction": "flying magical animal"}
    {"id": "4", "direction": "sea creatures"}
]
\end{verbatim}
- New Exploration Log: robot

\textbf{Output:} None
\end{prompt}

\section{Context-Adaptive Reuse}

\subsection{Block-level Adaptive Reuse}
Block-level adaptive reuse reuses the same direction from a previously explored block in a new context. This is implemented by passing the previously explored direction along with the updated design context (i.e., new design topic and current settings) into the suggestion generation pipeline described in Section~\ref{supp:suggestion}. No additional prompt is required for this reuse mechanism.


\subsection{Path-level Adaptive Reuse}\label{supp:pathlevel}

\begin{prompt}
\obeylines
\setlength{\parindent}{0pt}
\textbf{Prompt Instruction:}

Integrate pre-explored aspects with desired replication paths to create a tailored design exploration path. You have the explored aspects and the paths to be replicated, formatted in JSON structure. Your task is to suggest three coherent paths by marrying explored insights with replication goals, ensuring each suggestion aligns with previously explored directions and novelties. The three paths should be different from each other.

\# Steps:
1. Analyze the Pre-Explored Aspects and Replication Paths to identify connections and alignment.
2. Maintain the original IDs and properties from the Replication Paths while modifying their direction based on explored aspects.
3. Ensure three levels of variation:
- Path 1: Closest to the original direction.
- Path 2: Moderately evolved.
- Path 3: Highly tailored to the pre-explored aspects
4. Keep outputs abstract and structured, avoiding excessive specificity.

\# Output Format:
\begin{verbatim}
[
  {
    "id": "X",
    "property": "Property Name",
    "direction": "Updated Direction",
    "novelty": N
  },
  ...
]
\end{verbatim}
- ID: Must match the original Replication Path ID.
- Property: Must match the original property name.
- Direction: Adapted direction integrating Pre-Explored Aspects.
- Novelty: Adjusted novelty level reflecting changes.

\# Notes:
- Maintain abstraction of the direction; avoid unnecessary details. This direction will be used for further exploration, so make it shorter to foster wider exploration.
- Three paths should progressively increase in variation from the original.
- All three paths should be significantly different from each other.
- Keep responses concise and structured in JSON format.
- Consistency in IDs is crucial for traceability and validation of suggestions against original paths.

\vspace{0.5em}
\noindent\hrulefill
\vspace{0.5em}

\textbf{Examples:}

\textbf{Input:}
Design Topic: A professional character for a laboratory

Pre-Explored Aspects:
\begin{verbatim}
[
    {
        “id”: “9",
        “property”: “Character Entity”,
        “direction”: “Fluffy animal”,
        “novelty”: 1,
        “options”: [“Bear”, “Rabbit”, “Puppy”, “Raccoon”]
    }
]
\end{verbatim}

Replication Paths:
\begin{verbatim}
[
    {
        “id”: “2",
        “property”: “Laboratory Setting”,
        “direction”: “Computer”,
        “novelty”: 3
    },
    {
        “id”: “3",
        “property”: “Color Scheme”,
        “direction”: “professional blue”,
        “novelty”: 1
    }
]
\end{verbatim}

\textbf{Output:}
\begin{verbatim}
[
  [
    {
      "id": "2",
      "property": "Laboratory Setting",
      "direction": "Tech-savvy computer lab",
      "novelty": 3
    },
    {
      "id": "3",
      "property": "Color Scheme",
      "direction": "Professional Blue",
      "novelty": 1
    }
  ],
  [
    {
      "id": "2",
      "property": "Laboratory Setting",
      "direction": "Friendly computer workspace",
      "novelty": 3
    },
    {
      "id": "3",
      "property": "Color Scheme",
      "direction": "Cool Blue with Silver",
      "novelty": 2
    }
  ],
  [
    {
      "id": "2",
      "property": "Laboratory Setting",
      "direction": "Zoo Laboratory",
      "novelty": 3
    },
    {
      "id": "3",
      "property": "Color Scheme",
      "direction": "Green and Wood",
      "novelty": 2
    }
  ]
]
\end{verbatim}

\textbf{Input:}
Design Topic: A lovely animal character for a sports team

Pre-Explored Aspects:
\begin{verbatim}
[
    {
        "property": "Character Entity",
        "direction": "Bear",
        "novelty": 2,
        "options": ["Giant Panda", "Sloth Bear"]
    },
    {
        "property": "Character's Pose",
        "direction": "basketball",
        "novelty": 3,
        "options": ["Running the track",
                    "Half-Court Scrimmage",
                    "Shooting Practice"]
    }
]
\end{verbatim}

Replication Paths:
\begin{verbatim}
[
    {
        "id": "5",
        "property": "Image Style",
        "direction": "Pop Art",
        "novelty": 3
    },
    {
        "id": "9",
        "property": "Background or Setting",
        "direction": "stadium",
        "novelty": 4
    },
    {
        "id": "9_copy",
        "property": "Background or Setting",
        "direction": "training",
        "novelty": 5
    }
]
\end{verbatim}

\textbf{Output:}
\begin{verbatim}
[
  [
    {
      "id": "5",
      "property": "Image Style",
      "direction": "Colorful Pop Art",
      "novelty": 3
    },
    {
      "id": "9",
      "property": "Background or Setting",
      "direction": "Vibrant Stadium",
      "novelty": 4
    },
    {
      "id": "9_copy",
      "property": "Background or Setting",
      "direction": "Training Camp",
      "novelty": 5
    }
  ],
  [
    {
      "id": "5",
      "property": "Image Style",
      "direction": "Retro Pop Art",
      "novelty": 3
    },
    {
      "id": "9",
      "property": "Background or Setting",
      "direction": "Basketball Arena",
      "novelty": 4
    },
    {
      "id": "9_copy",
      "property": "Background or Setting",
      "direction": "Gym",
      "novelty": 5
    }
  ],
  [
    {
      "id": "5",
      "property": "Image Style",
      "direction": "Sporty Pop Art",
      "novelty": 3
    },
    {
      "id": "9",
      "property": "Background or Setting",
      "direction": "Basketball Field",
      "novelty": 4
    },
    {
      "id": "9_copy",
      "property": "Background or Setting",
      "direction": "Basketball training",
      "novelty": 5
    }
  ]
]
\end{verbatim}

\textbf{Input:}
Design Topic: An illustration for a child book cover with a friendly monster

Pre-Explored Aspects:
\begin{verbatim}
[
    {
        "id": "3",
        "property": "Monster's Appearance",
        "direction": "Jelly-like",
        "novelty": 3,
        "options": [
            "Velvet-like with a rich, deep hue",
            "Jelly-like, vibrant smile",
            "Cloth-like surface with sewn patterns",
            "Glossy, smooth surface"
        ]
    }
]

\end{verbatim}

Replication Paths:
\begin{verbatim}
[
    {
        "id": "7",
        "property": "Friendly Expression",
        "direction": "sticking out the tongue",
        "novelty": 2
    },
    {
        "id": "8",
        "property": "Background Setting",
        "direction": "fantasy playground",
        "novelty": 3
    },
    {
        "id": "11",
        "property": "Background Setting",
        "direction": "floating islands",
        "novelty": 2
    },
    {
        "id": "12",
        "property": "Child Character",
        "direction": "Small smiling kid",
        "novelty": 1
    }
]

\end{verbatim}

\textbf{Output:}
\begin{verbatim}
[
  [
    {
      "id": "7",
      "property": "Friendly Expression",
      "direction": "Cheerful Tongue Out",
      "novelty": 2
    },
    {
      "id": "8",
      "property": "Background Setting",
      "direction": "Whimsical Playground",
      "novelty": 3
    },
    {
      "id": "11",
      "property": "Background Setting",
      "direction": "Floating Island Adventure",
      "novelty": 2
    },
    {
      "id": "12",
      "property": "Child Character",
      "direction": "Joyful Child",
      "novelty": 1
    }
  ],
  [
    {
      "id": "7",
      "property": "Friendly Expression",
      "direction": "Playful Tongue Out",
      "novelty": 2
    },
    {
      "id": "8",
      "property": "Background Setting",
      "direction": "Mysterious Playground",
      "novelty": 3
    },
    {
      "id": "11",
      "property": "Background Setting",
      "direction": "Mystical Floating Lands",
      "novelty": 3
    },
    {
      "id": "12",
      "property": "Child Character",
      "direction": "Curious Kid",
      "novelty": 1
    }
  ],
  [
    {
      "id": "7",
      "property": "Friendly Expression",
      "direction": "Goofy grin with tongue out",
      "novelty": 2
    },
    {
      "id": "8",
      "property": "Background Setting",
      "direction": "Mysterious Playground",
      "novelty": 3
    },
    {
      "id": "11",
      "property": "Background Setting",
      "direction": "Enchanted Forest",
      "novelty": 3
    },
    {
      "id": "12",
      "property": "Child Character",
      "direction": "Scared Child",
      "novelty": 1
    }
  ]
]
\end{verbatim}

\textbf{Input:}
Design Topic: A scene of surreal worlds with fantasy mood

Pre-Explored Aspects:
\begin{verbatim}
[
    {
        "id": "3",
        "property": "Environmental Elements",
        "direction": "Upside-down waterfalls",
        "novelty": 3,
        "options": [
            "Skyward streams forming luminous bridges",
            "Waterfalls rising to meet the sun",
            "Water cascading upwards into the sky",
            "Reverse falls creating sky-bound rivers"
        ]
    }
]
\end{verbatim}

Replication Paths:
\begin{verbatim}
[
    {
        "id": "5",
        "property": "Color & Texture",
        "direction": "Vibrant",
        "novelty": 2
    },
    {
        "id": "8",
        "property": "Surreal Architecture",
        "direction": "Floating towers",
        "novelty": 2
    },
    {
        "id": "9",
        "property": "Surreal Architecture",
        "direction": "crystal palace",
        "novelty": 1
    }
]

\end{verbatim}

\textbf{Output:}
\begin{verbatim}
[
  [
    {
      "id": "5",
      "property": "Color & Texture",
      "direction": "Vibrant with Luminous Highlights",
      "novelty": 3
    },
    {
      "id": "8",
      "property": "Surreal Architecture",
      "direction": "Floating Towers",
      "novelty": 3
    },
    {
      "id": "9",
      "property": "Surreal Architecture",
      "direction": "Crystalline Palace",
      "novelty": 2
    }
  ],
  [
    {
      "id": "5",
      "property": "Color & Texture",
      "direction": "Vivid and Textured",
      "novelty": 3
    },
    {
      "id": "8",
      "property": "Surreal Architecture",
      "direction": "Floating Coral Towers",
      "novelty": 3
    },
    {
      "id": "9",
      "property": "Surreal Architecture",
      "direction": "Crystal Oasis Palace",
      "novelty": 2
    }
  ],
  [
    {
      "id": "5",
      "property": "Color & Texture",
      "direction": "Vibrant Neon Green",
      "novelty": 3
    },
    {
      "id": "8",
      "property": "Surreal Architecture",
      "direction": "Mystical Floating Towers",
      "novelty": 3
    },
    {
      "id": "9",
      "property": "Surreal Architecture",
      "direction": "Water Palace",
      "novelty": 2
    }
  ]
]
\end{verbatim}

\textbf{Input:}
Design Topic: A futuristic mascot for an AI startup

Pre-Explored Aspects:
\begin{verbatim}
[
    {
        "property": "Mascot's Entity",
        "direction": "Simple shape",
        "novelty": 3,
        "options": ["Geometric Circle", "Triangular Prism", "Abstract Cube"]
    },
    {
        "property": "Futuristic Background",
        "direction": "VR",
        "novelty": 2,
        "options": [
            "Virtual Cityscape",
            "Futuristic Control Room",
            "Immersive Forest Path",
            "Cyberpunk Alleyway"
        ]
    }
]

\end{verbatim}

Replication Paths:
\begin{verbatim}
[
    {
        "id": "43",
        "property": "Image Style",
        "direction": "Watercolor illustration",
        "novelty": 1
    },
    {
        "id": "46",
        "property": "Mascot's Pose",
        "direction": "friendly",
        "novelty": 2
    },
    {
        "id": "49",
        "property": "Mascot's Pose",
        "direction": "working",
        "novelty": 4
    },
    {
        "id": "47",
        "property": "Background or Setting",
        "direction": "outdoor",
        "novelty": 3
    }
]


\end{verbatim}

\textbf{Output:}
\begin{verbatim}
[
  [
    {
      "id": "43",
      "property": "Image Style",
      "direction": "Digital Watercolor with Geometric Patterns",
      "novelty": 2
    },
    {
      "id": "46",
      "property": "Mascot's Pose",
      "direction": "Friendly and Inviting",
      "novelty": 2
    },
    {
      "id": "49",
      "property": "Mascot's Pose",
      "direction": "Engaged in Task",
      "novelty": 4
    },
    {
      "id": "47",
      "property": "Background or Setting",
      "direction": "Virtual Outdoor Space",
      "novelty": 3
    }
  ],
  [
    {
      "id": "43",
      "property": "Image Style",
      "direction": "Minimalist Watercolor",
      "novelty": 2
    },
    {
      "id": "46",
      "property": "Mascot's Pose",
      "direction": "Welcoming Gesture",
      "novelty": 2
    },,
    {
      "id": "49",
      "property": "Mascot's Pose",
      "direction": "Collaborative Stance",
      "novelty": 4
    },
    {
      "id": "47",
      "property": "Background or Setting",
      "direction": "Futuristic Outdoor Scene",
      "novelty": 3
    }
  ],
  [
    {
      "id": "43",
      "property": "Image Style",
      "direction": "Evocative Watercolor",
      "novelty": 2
    },
    {
      "id": "46",
      "property": "Mascot's Pose",
      "direction": "Expressively Friendly",
      "novelty": 2
    },
    {
      "id": "49",
      "property": "Mascot's Pose",
      "direction": "Dynamic and Focused",
      "novelty": 4
    },
    {
      "id": "47",
      "property": "Background or Setting",
      "direction": "Cybernetic Outdoor Setting",
      "novelty": 3
    }
  ]
]
\end{verbatim}
\end{prompt}

\subsection{Project-level Adaptive Reuse}

\begin{prompt}
\obeylines
\setlength{\parindent}{0pt}
\textbf{Prompt Instruction:}

User is exploring different ideas for their graphic design project, and wants to refer to their previous exploration pattern for their new design project. You will be given the explored aspects and the paths to be replicated, formatted in JSON structure. Your task is to generate three coherent paths by marrying previously explored insights with a new design project topic, ensuring each suggestion aligns with previously explored directions and novelties. The three paths should be different from each other.

\# Steps:
1. Analyze the user's past exploration path to identify their exploration pattern.
2. Maintain the original IDs and properties from the past exploration path while modifying their direction based on the newly given topic.
3. Ensure three levels of variation:
- Path 1: Closest to the original path. In this path, if the original design topic and the new design topic are similar, you can use the same direction.
- Path 2: Moderately evolved.
- Path 3: Highly tailored to the new topic.
4. Avoid making outputs too specific or too long. Do not use abstract terms, but do not make the overall concept too specific. Keep the specificity same with the original.

\# Output Format:
\begin{verbatim}
[
  {
    "id": "X",
    "property": "Property Name",
    "direction": "Updated Direction",
    "novelty": N
  },
  ...
]
\end{verbatim}
- ID: Must match the original Replication Path ID.
- Property: Must match the original property name.
- Direction: Adapted direction integrating the new design topic.
- Novelty: Adjusted novelty level reflecting changes.

\# Notes:
- Maintain abstraction when generating variations. Match the level of abstraction in the Previous Exploration History. Do not make the new direction more detailed or specific than the original.
  -- Example: if the original direction is ``animal'' (abstract), a valid variation is ``plant'' (similarly abstract). An invalid variation would be ``cactus'' (too specific).
- Three paths should progressively increase in variation from the original.
- All three paths should be significantly different from each other.
- Keep responses concise and structured in JSON format.
- Consistency in IDs is crucial for traceability and validation of suggestions against original paths.

\vspace{0.5em}
\noindent\hrulefill
\vspace{0.5em}

\textbf{Examples:}

\textbf{Input:}
Original Design Topic: A cute character for a baseball team

Previous Exploration History:
\begin{verbatim}
[
    {
        "id": "9",
        "property": "Character Entity",
        "direction": "Fluffy animal",
        "novelty": 1
    }
]
\end{verbatim}

New Design Topic: A professional character for a laboratory

\textbf{Output:}
\begin{verbatim}
[
  [
    {
      "id": "9",
      "property": "Character Entity",
      "direction": "Round-shaped Animal",
      "novelty": 1
    }
  ],
  [
    {
      "id": "9",
      "property": "Character Entity",
      "direction": "Sleek Animal",
      "novelty": 1
    }
  ],
  [
    {
      "id": "9",
      "property": "Character Entity",
      "direction": "Anthropomorphic scientist",
      "novelty": 2
    }
  ]
]
\end{verbatim}

\textbf{Input:}
Original Design Topic: A lovely animal character for a sports team

Previous Exploration History:
\begin{verbatim}
[
    {
        "id": "5",
        "property": "Image Style",
        "direction": "Pop Art",
        "novelty": 3
    },
    {
        "id": "9",
        "property": "Background or Setting",
        "direction": "stadium",
        "novelty": 4
    },
    {
        "id": "9_copy",
        "property": "Background or Setting",
        "direction": "training",
        "novelty": 5
    }
]
\end{verbatim}

New Design Topic: A mascot character for an environmental-friendly company

\textbf{Output:}
\begin{verbatim}
[
  [
    {
      "id": "5",
      "property": "Image Style",
      "direction": "Pop Art",
      "novelty": 3
    },
    {
      "id": "9",
      "property": "Background or Setting",
      "direction": "forest",
      "novelty": 4
    },
    {
      "id": "9_copy",
      "property": "Background or Setting",
      "direction": "working",
      "novelty": 5
    }
  ],
  [
    {
      "id": "5",
      "property": "Image Style",
      "direction": "Flat Design",
      "novelty": 4
    },
    {
      "id": "9",
      "property": "Background or Setting",
      "direction": "garden",
      "novelty": 4
    },
    {
      "id": "9_copy",
      "property": "Background or Setting",
      "direction": "working",
      "novelty": 5
    }
  ],
  [
    {
      "id": "5",
      "property": "Image Style",
      "direction": "Eco Minimalist",
      "novelty": 5
    },
    {
      "id": "9",
      "property": "Background or Setting",
      "direction": "urban green rooftop",
      "novelty": 5
    },
    {
      "id": "9_copy",
      "property": "Background or Setting",
      "direction": "recycling",
      "novelty": 5
    }
  ]
]
\end{verbatim}

\textbf{Input:}
Original Design Topic: An illustration for a child book cover with a friendly monster

Previous Exploration History:
\begin{verbatim}
[
    {
        "id": "7",
        "property": "Facial Expression",
        "direction": "sticking out the tongue",
        "novelty": 2
    },
    {
        "id": "8",
        "property": "Background Setting",
        "direction": "playground",
        "novelty": 3
    },
    {
        "id": "11",
        "property": "Background Setting",
        "direction": "floating islands",
        "novelty": 2
    },
    {
        "id": "12",
        "property": "Character Entity",
        "direction": "Small smiling kid",
        "novelty": 1
    }
]
\end{verbatim}

New Design Topic: A scene of surreal worlds with fantasy mood

\textbf{Output:}
\begin{verbatim}
[
  [
    {
      "id": "7",
      "property": "Facial Expression",
      "direction": "grinning widely",
      "novelty": 2
    },
    {
      "id": "8",
      "property": "Background Setting",
      "direction": "magical playground",
      "novelty": 3
    },
    {
      "id": "11",
      "property": "Background Setting",
      "direction": "floating islands",
      "novelty": 2
    },
    {
      "id": "12",
      "property": "Character Entity",
      "direction": "Tiny creature",
      "novelty": 1
    }
  ],
  [
    {
      "id": "7",
      "property": "Facial Expression",
      "direction": "amazed wonder",
      "novelty": 3
    },
    {
      "id": "8",
      "property": "Background Setting",
      "direction": "dreamlike garden",
      "novelty": 4
    },
    {
      "id": "11",
      "property": "Background Setting",
      "direction": "cloud",
      "novelty": 3
    },
    {
      "id": "12",
      "property": "Character Entity",
      "direction": "Curious animal",
      "novelty": 2
    }
  ],
  [
    {
      "id": "7",
      "property": "Facial Expression",
      "direction": "mysterious smile",
      "novelty": 4
    },
    {
      "id": "8",
      "property": "Background Setting",
      "direction": "labyrinth",
      "novelty": 5
    },
    {
      "id": "11",
      "property": "Background Setting",
      "direction": "fractured",
      "novelty": 5
    },
    {
      "id": "12",
      "property": "Character Entity",
      "direction": "Surreal shape",
      "novelty": 4
    }
  ]
]
\end{verbatim}

\textbf{Input:}
Original Design Topic: A futuristic mascot for an AI startup

Previous Exploration History:
\begin{verbatim}
[
    {
        "id": "43",
        "property": "Image Style",
        "direction": "Watercolor illustration",
        "novelty": 1
    },
    {
        "id": "46",
        "property": "Mascot's Pose",
        "direction": "friendly",
        "novelty": 2
    },
    {
        "id": "49",
        "property": "Mascot's Pose",
        "direction": "working",
        "novelty": 4
    },
    {
        "id": "47",
        "property": "Background or Setting",
        "direction": "outdoor",
        "novelty": 3
    }
]
\end{verbatim}

New Design Topic: A friendly mascot for a hamburger restaurant

\textbf{Output:}
\begin{verbatim}
[
  [
    {
      "id": "43",
      "property": "Image Style",
      "direction": "Watercolor illustration",
      "novelty": 1
    },
    {
      "id": "46",
      "property": "Mascot's Pose",
      "direction": "friendly",
      "novelty": 2
    },
    {
      "id": "49",
      "property": "Mascot's Pose",
      "direction": "serving",
      "novelty": 4
    },
    {
      "id": "47",
      "property": "Background or Setting",
      "direction": "outdoor",
      "novelty": 3
    }
  ],
  [
    {
      "id": "43",
      "property": "Image Style",
      "direction": "Flat illustration",
      "novelty": 2
    },
    {
      "id": "46",
      "property": "Mascot's Pose",
      "direction": "inviting",
      "novelty": 3
    },
    {
      "id": "49",
      "property": "Mascot's Pose",
      "direction": "welcoming",
      "novelty": 4
    },
    {
      "id": "47",
      "property": "Background or Setting",
      "direction": "diner interior",
      "novelty": 4
    }
  ],
  [
    {
      "id": "43",
      "property": "Image Style",
      "direction": "Retro cartoon",
      "novelty": 4
    },
    {
      "id": "46",
      "property": "Mascot's Pose",
      "direction": "dynamic action",
      "novelty": 4
    },
    {
      "id": "49",
      "property": "Mascot's Pose",
      "direction": "juggling food",
      "novelty": 5
    },
    {
      "id": "47",
      "property": "Background or Setting",
      "direction": "city street",
      "novelty": 4
    }
  ]
]
\end{verbatim}
\end{prompt}


\section{System-generated Direction Recommendations}\label{appendix:prompt4}

\begin{prompt}
\obeylines
\setlength{\parindent}{0pt}
\textbf{Prompt Instruction:}

Provide two design ideas based on a given topic and property, considering the exploration history and current settings. Your goal is to deliver a typical and unique recommendation for the given property to aid the designer’s exploration of diverse ideas.

\# You will receive:
- Design Topic: The main subject of the whole design exploration
- Property Name: The specific attribute or element of the design that needs to be explored now
- Exploration History: A summary of what the designer has explored related to the property so far
- Current Setting: The designer's current idea or approach that has been set. This can contain information that is not about the current property.

\# Generate two different recommendations:
- Typical recommendation: closely related to the exploration history and current settings
- Unique recommendation: loosely related to the exploration history and current settings

\# Notes:
- Avoid suggestions that have already been covered in the exploration history.
- Suggestions should be high-level and vague so that users can think more about them.
- Avoid too narrow and specific suggestions, as it can hurt the user's broad exploration.
- Suggestions should be short and concise, less than 3 words.

\vspace{0.5em}
\noindent\hrulefill
\vspace{0.5em}

\textbf{Examples:}

\textbf{Input:}
- Design Topic: A professional character for a laboratory
- Property Name: Image Style
- Exploration History: []
- Current Setting: ["Character Entity: Robot"]

\textbf{Output:}
\begin{verbatim}
{
  "typical": "Realistic",
  "unique": "Steampunk"
}
\end{verbatim}

\textbf{Input:}
- Design Topic: A lovely animal character for a baseball team
- Property Name: Character Pose
- Exploration History: ["Baseball-related pose"]
- Current Setting: ["Character Entity: Fluffy animal", "Team Color: Blue"]

\textbf{Output:}
\begin{verbatim}
{
  "typical": "Ball-related",
  "unique": "Cheerleading"
}
\end{verbatim}

\textbf{Input:}
- Design Topic: An illustration for a child book cover with a friendly monster
- Property Name: Illustration Style
- Exploration History: ["Minimalistic", "Line drawing"]
- Current Setting: ["Monster's Appearance: Fluffy and Circular shape"]

\textbf{Output:}
\begin{verbatim}
{
  "typical": "Watercolor",
  "unique": "Retro cartoon"
}
\end{verbatim}

\textbf{Input:}
- Design Topic: A scene of surreal worlds with fantasy mood
- Property Name: Surreal Architecture
- Exploration History: []
- Current Setting: ["Environmental Elements: Floating Islands", "Color \& Texture: Pastel"]

\textbf{Output:}
\begin{verbatim}
{
  "typical": "Twisting buildings",
  "unique": "Giant seashell"
}
\end{verbatim}
\end{prompt}
